Searching for Topological Symmetry in Data Haystack

Finding interesting symmetrical topological structures in high-dimensional systems is an important problem in statistical machine learning. Limited amount of available high-dimensional data and its sensitivity to noise pose computational challenges to find symmetry. Our paper presents a new method to find local symmetries in a low-dimensional 2-D grid structure which is embedded in high-dimensional structure. To compute the symmetry in a grid structure, we introduce three legal grid moves (i) Commutation (ii) Cyclic Permutation (iii) Stabilization on sets of local grid squares, grid blocks. The three grid moves are legal transformations as they preserve the statistical distribution of hamming distances in each grid block. We propose and coin the term of grid symmetry of data on the 2-D data grid as the invariance of statistical distributions of hamming distance are preserved after a sequence of grid moves. We have computed and analyzed the grid symmetry of data on multivariate Gaussian distributions and Gamma distributions with noise.

==> tikzlibraryknots.code.tex <==
%%
%% This is file `tikzlibraryknots.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% spath3.dtx  (with options: `knots')
%% ----------------------------------------------------------------
%% spath3 --- Functions for manipulating PGF soft paths
%% E-mail: stacey@math.ntnu.no
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
%%
\RequirePackage{spath3}
\usetikzlibrary{intersections}

\ExplSyntaxOn

\tl_new:N \l__knot_tmpa_tl
\tl_new:N \l__knot_tmpb_tl
\tl_new:N \l__knot_tmpc_tl
\tl_new:N \l__knot_tmpd_tl
\tl_new:N \l__knot_tmpe_tl
\tl_new:N \l__knot_tmpf_tl
\tl_new:N \l__knot_tmpg_tl
\tl_new:N \l__knot_redraws_tl
\tl_new:N \l__knot_clip_width_tl
\tl_new:N \l__knot_name_tl
\tl_new:N \l__knot_node_tl

\int_new:N \l__knot_tmpa_int
\int_new:N \l__knot_strands_int
\int_new:N \l__knot_intersections_int
\int_new:N \l__knot_filaments_int
\int_new:N \l__knot_component_start_int

\dim_new:N \l__knot_tmpa_dim
\dim_new:N \l__knot_tmpb_dim
\dim_new:N \l__knot_tmpc_dim
\dim_new:N \l__knot_tolerance_dim
\dim_new:N \l__knot_clip_radius_dim

\bool_new:N \l__knot_draft_bool
\bool_new:N \l__knot_ignore_ends_bool
\bool_new:N \l__knot_self_intersections_bool
\bool_new:N \l__knot_splits_bool
\bool_new:N \l__knot_super_draft_bool

\bool_new:N \l__knot_prepend_prev_bool
\bool_new:N \l__knot_append_next_bool
\bool_new:N \l__knot_skip_bool

\bool_set_true:N \l__knot_ignore_ends_bool
\tikzset{
  knot/.code={
    \tl_if_eq:nnTF {#1} {none}
    {
      \tikz@addmode{\tikz@mode@doublefalse}
    }
    {
      \tikz@addmode{\tikz@mode@doubletrue}
      \tl_if_eq:nnTF {\pgfkeysnovalue} {#1}
      {
        \tikz@addoption{\pgfsetinnerstrokecolor{.}}
      }
      {
        \pgfsetinnerstrokecolor{#1}
      }
      \tikz@addoption{
        \pgfsetstrokecolor{knotbg}
      }
      \tl_set:Nn \tikz@double@setup{
        \pgfsetinnerlinewidth{\pgflinewidth}
        \pgfsetlinewidth{\dim_eval:n {\tl_use:N \l__knot_gap_tl \pgflinewidth}}
      }
    }
  },
  knot~ gap/.store~ in=\l__knot_gap_tl,
  knot~ gap=3,
  knot~ diagram/.is~family,
  knot~ diagram/.unknown/.code={
    \tl_set_eq:NN \l__knot_tmpa_tl \pgfkeyscurrentname
    \pgfkeysalso{
      /tikz/\l__knot_tmpa_tl=#1
    }
  },
  background~ colour/.code={%
    \colorlet{knotbg}{#1}%
  },
  background~ color/.code={%
    \colorlet{knotbg}{#1}%
  },
  background~ colour=white,
  knot~ diagram,
  name/.store~in=\l__knot_name_tl,
  name={knot},
  every~ strand/.style={draw},
  ignore~ endpoint~ intersections/.code={
    \tl_if_eq:nnTF {#1} {true}
    {
      \bool_set_true:N \l__knot_ignore_ends_bool
    }
    {
      \bool_set_false:N \l__knot_ignore_ends_bool
    }
  },
  ignore~ endpoint~ intersections/.default=true,
  consider~ self~ intersections/.is~choice,
  consider~ self~ intersections/true/.code={
    \bool_set_true:N \l__knot_self_intersections_bool
    \bool_set_true:N \l__knot_splits_bool
  },
  consider~ self~ intersections/false/.code={
    \bool_set_false:N \l__knot_self_intersections_bool
    \bool_set_false:N \l__knot_splits_bool
  },
  consider~ self~ intersections/no~ splits/.code={
    \bool_set_true:N \l__knot_self_intersections_bool
    \bool_set_false:N \l__knot_splits_bool
  },
  consider~ self~ intersections/.default={true},
  clip~ radius/.code={
    \dim_set:Nn \l__knot_clip_radius_dim {#1}
  },
  clip~ radius=10pt,
  end~ tolerance/.code={
    \dim_set:Nn \l__knot_tolerance_dim {#1}
  },
  end~ tolerance=14pt,
  clip~ width/.code={
    \tl_set:Nn \l__knot_clip_width_tl {#1}
  },
  clip~ width=3,
  flip~ crossing/.code={%
    \tl_clear_new:c {l__knot_crossing_#1}
    \tl_set:cn {l__knot_crossing_#1} {x}
  },
  draft~ mode/.is~ choice,
  draft~ mode/off/.code={%
    \bool_set_false:N \l__knot_draft_bool
    \bool_set_false:N \l__knot_super_draft_bool
  },
  draft~ mode/crossings/.code={%
    \bool_set_true:N \l__knot_draft_bool
    \bool_set_false:N \l__knot_super_draft_bool
  },
  draft~ mode/strands/.code={%
    \bool_set_true:N \l__knot_draft_bool
    \bool_set_true:N \l__knot_super_draft_bool
  },
  draft/.is~ family,
  draft,
  crossing~ label/.style={
    overlay,
    fill=white,
    fill~ opacity=.5,
    text~ opacity=1,
    text=blue,
    pin~ edge={blue,<-}
  },
  strand~ label/.style={
    overlay,
    circle,
    draw=purple,
    fill=white,
    fill~ opacity=.5,
    text~ opacity=1,
    text=purple,
    inner~ sep=0pt
  },
}
\cs_new_nopar:Npn \knot_apply_style:N #1
{
  \tl_if_exist:NT #1 {
    \exp_args:NV \tikzset #1
  }
}
\cs_generate_variant:Nn \knot_apply_style:N {c}
\NewDocumentCommand \flipcrossings {m}
{
  \tikzset{knot~ diagram/flip~ crossing/.list={#1}}%
}
\NewDocumentCommand \strand { O{} }
{
  \int_incr:N \l__knot_strands_int
  \tl_clear_new:c {l__knot_options_strand \int_use:N \l__knot_strands_int}
  \tl_set:cn {l__knot_options_strand \int_use:N \l__knot_strands_int} {#1}
  \path[#1,save~ spath=knot strand \int_use:N  \l__knot_strands_int]
}
\NewDocumentEnvironment{knot} { O{} }
{
  \knot_initialise:n {#1}
}
{
  \knot_render:
}
\cs_new_protected_nopar:Npn \knot_initialise:n #1
{
  \tikzset{knot~ diagram/.cd,every~ knot~ diagram/.try,#1}
  \int_zero:N \l__knot_strands_int
  \tl_clear:N \l__knot_redraws_tl
}
\cs_new_protected_nopar:Npn \knot_render:
{
  \pgfscope
  \pgftransformreset
  \int_step_function:nnnN {1} {1} {\l__knot_strands_int} \knot_draw_strand:n
  \bool_if:NF \l__knot_super_draft_bool
  {
    \int_step_function:nnnN {1} {1} {\l__knot_strands_int} \knot_draw_labels:n
    \bool_if:NTF \l__knot_self_intersections_bool
    {
      \knot_split_strands:
      \int_set_eq:NN \l__knot_tmpa_int \l__knot_filaments_int
      \tl_set:Nn \l__knot_prefix_tl {filament}
    }
    {
      \int_set_eq:NN \l__knot_tmpa_int \l__knot_strands_int
      \tl_set:Nn \l__knot_prefix_tl {strand}
    }
    \int_gzero:N \l__knot_intersections_int
    \bool_if:NTF \l__knot_draft_bool
    {
      \tl_set:Nn \l__knot_node_tl
      {\node[coordinate,pin={[knot~ diagram/draft/crossing~ label]{\int_use:N \l__knot_intersections_int}}]}
    }
    {
      \tl_set:Nn \l__knot_node_tl {\node[coordinate]}
    }
    \int_step_variable:nnnNn {1} {1} {\l__knot_tmpa_int - 1} \l__knot_tmpa_tl
    {
      \int_step_variable:nnnNn {\tl_use:N \l__knot_tmpa_tl + 1} {1}     {\l__knot_tmpa_int} \l__knot_tmpb_tl
      {
        \knot_intersections:VV \l__knot_tmpa_tl \l__knot_tmpb_tl
      }
    }
    \tl_use:N \l__knot_redraws_tl
  }
  \endpgfscope
}
\cs_new_protected_nopar:Npn \knot_draw_strand:n #1
{
  \pgfscope
  \group_begin:
  \tl_set:Nn \l_tmpa_tl {knot~ diagram/every~ strand/.try,}
  \tl_put_right:Nv \l_tmpa_tl {l__knot_options_strand #1}
  \tl_put_right:Nn \l_tmpa_tl {,knot~ diagram/only~ when~ rendering/.try,only~ when~ rendering/.try}
  \spath_bake_round:n {knot strand #1}
  \spath_tikz_path:Vn \l_tmpa_tl {knot strand #1}
  \group_end:
  \endpgfscope
}
\cs_generate_variant:Nn \tl_put_right:Nn {Nv}
\cs_new_protected_nopar:Npn \knot_draw_labels:n #1
{
  \bool_if:NT \l__knot_draft_bool
  {
    \spath_get:nnN {knot strand #1} {final point} \l__knot_tmpb_tl
    \dim_set:Nn \l__knot_tmpa_dim {\tl_item:Nn \l__knot_tmpb_tl {1}}
    \dim_set:Nn \l__knot_tmpb_dim {\tl_item:Nn \l__knot_tmpb_tl {2}}
    \node[knot~ diagram/draft/strand~label] at (\l__knot_tmpa_dim,\l__knot_tmpb_dim) {#1};
    \spath_get:nnN {knot strand #1} {initial point} \l__knot_tmpb_tl
    \dim_set:Nn \l__knot_tmpa_dim {\tl_item:Nn \l__knot_tmpb_tl {1}}
    \dim_set:Nn \l__knot_tmpb_dim {\tl_item:Nn \l__knot_tmpb_tl {2}}
    \node[knot~ diagram/draft/strand~label] at (\l__knot_tmpa_dim,\l__knot_tmpb_dim) {#1};
  }
  \bool_if:nT {
    \l__knot_self_intersections_bool
    &&
    \l__knot_splits_bool
  }
  {
    \tl_clear:N \l__knot_tmpa_tl
    \spath_map_segment_function:nN {knot strand #1} \knot_split_self_intersects:NN
    \spath_put:nnV {knot strand #1} {path} \l__knot_tmpa_tl
  }
}
\cs_new_protected_nopar:Npn \knot_split_self_intersects:NN #1#2
{
  \tl_case:NnF #1
  {
    \g__spath_curvetoa_tl
    {
      \fp_set:Nn \l_tmpa_fp
      {
        (\tl_item:Nn #2 {3} - 3 * \tl_item:Nn #2 {6} + 3 * \tl_item:Nn #2 {9} - \tl_item:Nn #2 {12})
        *
        (3 * \tl_item:Nn #2 {8} - 3 * \tl_item:Nn #2 {11})
        -
        (\tl_item:Nn #2 {2} - 3 * \tl_item:Nn #2 {5} + 3 * \tl_item:Nn #2 {8} - \tl_item:Nn #2 {11})
        *
        (3 * \tl_item:Nn #2 {9} - 3 * \tl_item:Nn #2 {12})
      }
      \fp_set:Nn \l_tmpb_fp
      {
        (\tl_item:Nn #2 {2} - 3 * \tl_item:Nn #2 {5} + 3 * \tl_item:Nn #2 {8} - \tl_item:Nn #2 {11})
        *
        (3 * \tl_item:Nn #2 {6} - 6 * \tl_item:Nn #2 {9} + 3 * \tl_item:Nn #2 {12})
        -
        (\tl_item:Nn #2 {3} - 3 * \tl_item:Nn #2 {6} + 3 * \tl_item:Nn #2 {9} - \tl_item:Nn #2 {12})
        *
        (3 * \tl_item:Nn #2 {5} - 6 * \tl_item:Nn #2 {8} + 3 * \tl_item:Nn #2 {11})
      }
      \fp_compare:nTF
      {
        \l_tmpb_fp != 0
      }
      {
        \fp_set:Nn \l_tmpa_fp {.5 * \l_tmpa_fp / \l_tmpb_fp}
        \fp_compare:nTF
        {
          0 < \l_tmpa_fp && \l_tmpa_fp < 1
        }
        {
          \spath_split_curve:VVNN \l_tmpa_fp #2 \l_tmpa_tl \l_tmpb_tl
          \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
          \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
          \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
          \tl_set:Nx \l_tmpb_tl {\tl_tail:N \l_tmpb_tl}
          \tl_set:Nx \l_tmpb_tl {\tl_tail:N \l_tmpb_tl}
          \tl_set:Nx \l_tmpb_tl {\tl_tail:N \l_tmpb_tl}
          \tl_put_right:NV \l__knot_tmpa_tl \l_tmpa_tl
          \tl_put_right:NV \l__knot_tmpa_tl \l_tmpb_tl
        }
        {
          \tl_set_eq:NN \l_tmpa_tl #2
          \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
          \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
          \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
          \tl_put_right:NV \l__knot_tmpa_tl \l_tmpa_tl
        }
      }
      {
        \tl_set_eq:NN \l_tmpa_tl #2
        \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
        \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
        \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
        \tl_put_right:NV \l__knot_tmpa_tl \l_tmpa_tl
      }
    }
    \g__spath_lineto_tl
    {
      \tl_set_eq:NN \l_tmpa_tl #2
      \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
      \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
      \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
      \tl_put_right:NV \l__knot_tmpa_tl \l_tmpa_tl
    }
  }
  {
    \tl_put_right:NV \l__knot_tmpa_tl #2
  }
}
\cs_new_protected_nopar:Npn \knot_intersections:nn #1#2
{
  \group_begin:
  \tl_set_eq:NN \l__knot_tmpa_tl \l__knot_prefix_tl
  \tl_put_right:Nn \l__knot_tmpa_tl {#1}
  \tl_set_eq:NN \l__knot_tmpb_tl \l__knot_prefix_tl
  \tl_put_right:Nn \l__knot_tmpb_tl {#2}
  \spath_get:nnN {knot \tl_use:N \l__knot_tmpa_tl} {path} \l__knot_tmpc_tl
  \spath_get:nnN {knot \tl_use:N \l__knot_tmpb_tl} {path} \l__knot_tmpd_tl

  \pgfintersectionofpaths{\pgfsetpath\l__knot_tmpc_tl}{\pgfsetpath\l__knot_tmpd_tl}

  \int_compare:nT {\pgfintersectionsolutions > 0}
  {
    \int_step_function:nnnN {1} {1} {\pgfintersectionsolutions} \knot_do_intersection:n
  }
  \group_end:
}
\cs_new_protected_nopar:Npn \knot_do_intersection:n #1
{
  \pgfpointintersectionsolution{#1}
  \dim_set:Nn \l__knot_tmpa_dim {\pgf@x}
  \dim_set:Nn \l__knot_tmpb_dim {\pgf@y}
  \bool_set_false:N \l__knot_skip_bool
  \bool_if:NT \l__knot_self_intersections_bool
  {
    \tl_set:Nn \l_tmpa_tl {knot previous}
    \tl_put_right:NV \l_tmpa_tl \l__knot_tmpa_tl
    \tl_set:Nv \l_tmpa_tl \l_tmpa_tl
    \tl_if_eq:NNT \l_tmpa_tl \l__knot_tmpb_tl
    {
      \knot_test_endpoint:VnT \l__knot_tmpb_tl {final point}
      {
        \bool_set_true:N \l__knot_skip_bool
      }
    }

    \tl_set:Nn \l_tmpa_tl {knot previous}
    \tl_put_right:NV \l_tmpa_tl \l__knot_tmpb_tl
    \tl_set:Nv \l_tmpa_tl \l_tmpa_tl
    \tl_if_eq:NNT \l_tmpa_tl \l__knot_tmpa_tl
    {
      \knot_test_endpoint:VnT \l__knot_tmpa_tl {final point}
      {
        \bool_set_true:N \l__knot_skip_bool
      }
    }
  }
  \bool_if:NT \l__knot_ignore_ends_bool
  {
    \knot_test_endpoint:VnT \l__knot_tmpa_tl {initial point}
    {
      \bool_set_true:N \l__knot_skip_bool
    }
    \knot_test_endpoint:VnT \l__knot_tmpa_tl {final point}
    {
      \bool_set_true:N \l__knot_skip_bool
    }
    \knot_test_endpoint:VnT \l__knot_tmpb_tl {initial point}
    {
      \bool_set_true:N \l__knot_skip_bool
    }
    \knot_test_endpoint:VnT \l__knot_tmpb_tl {final point}
    {
      \bool_set_true:N \l__knot_skip_bool
    }
  }
  \bool_if:NF \l__knot_skip_bool
  {

    \int_gincr:N \l__knot_intersections_int
    \bool_if:nTF
    {
      \tl_if_exist_p:c {l__knot_crossing_ \int_use:N
        \l__knot_intersections_int}
      &&
      ! \tl_if_empty_p:c {l__knot_crossing_ \int_use:N
        \l__knot_intersections_int}
    }
    {
      \tl_set_eq:NN \l__knot_tmpg_tl \l__knot_tmpb_tl
    }
    {
      \tl_set_eq:NN \l__knot_tmpg_tl \l__knot_tmpa_tl
    }
    \bool_if:NT \l__knot_self_intersections_bool
    {
      \knot_test_endpoint:VnT \l__knot_tmpg_tl {initial point}
      {
        \bool_set_true:N \l__knot_prepend_prev_bool
      }
      {
        \bool_set_false:N \l__knot_prepend_prev_bool
      }

      \knot_test_endpoint:VnT \l__knot_tmpg_tl {final point}
      {
        \bool_set_true:N \l__knot_append_next_bool
      }
      {
        \bool_set_false:N \l__knot_append_next_bool
      }
      \bool_if:nT
      {
        \l__knot_prepend_prev_bool || \l__knot_append_next_bool
      }
      {
        \spath_clone:nn {knot \tl_use:N \l__knot_tmpg_tl}
        {knot \tl_use:N \l__knot_prefix_tl -1}

        \tl_set_eq:cc {l__knot_options_ \tl_use:N \l__knot_prefix_tl -1} {l__knot_options_ \tl_use:N \l__knot_tmpg_tl}

        \bool_if:nT
        {
          \l__knot_prepend_prev_bool
          &&
          \tl_if_exist_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
          &&
          !\tl_if_empty_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
        }
        {
          \spath_prepend_no_move:nn {knot \tl_use:N \l__knot_prefix_tl -1} {knot \tl_use:c {knot previous \tl_use:N \l__knot_tmpg_tl}}
          \bool_if:nT
          {
            \l__knot_splits_bool
            &&
            \tl_if_exist_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
            &&
            !\tl_if_empty_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
          }
          {
            \knot_test_endpoint:vnT {knot previous \tl_use:N \l__knot_tmpg_tl} {initial point}
            {
              \spath_get:nnN {knot \tl_use:N \l__knot_prefix_tl -1} {path} \l_tmpa_tl
              \spath_prepend_no_move:nn {knot \tl_use:N \l__knot_prefix_tl -1} {knot \tl_use:c {knot previous \tl_use:c {knot previous \tl_use:N \l__knot_tmpg_tl}}}
              \spath_get:nnN {knot \tl_use:N \l__knot_prefix_tl -1} {path} \l_tmpa_tl

            }
          }
        }
        \bool_if:nT
        {
          \l__knot_append_next_bool
          &&
          \tl_if_exist_p:c {knot next \tl_use:N \l__knot_tmpg_tl}
          &&
          !\tl_if_empty_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
        }
        {
          \spath_append_no_move:nn {knot \tl_use:N \l__knot_prefix_tl -1} {knot \tl_use:c {knot next \tl_use:N \l__knot_tmpg_tl}}
          \bool_if:nT
          {
            \l__knot_splits_bool
            &&
            \tl_if_exist_p:c {knot previous \tl_use:N
              \l__knot_tmpg_tl}
            &&
            !\tl_if_empty_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
          }
          {
            \knot_test_endpoint:vnT {knot previous \tl_use:N \l__knot_tmpg_tl} {final point}
            {
              \spath_append_no_move:nn {knot \tl_use:N \l__knot_prefix_tl -1} {knot \tl_use:c {knot next \tl_use:c {knot next \tl_use:N \l__knot_tmpg_tl}}}

            }
          }
        }

        \tl_set:Nn \l__knot_tmpg_tl {\tl_use:N \l__knot_prefix_tl -1}
      }
    }
    \pgfscope
    \group_begin:
    \tikzset{knot~ diagram/every~ intersection/.try, every~ intersection/.try, knot~ diagram/intersection~ \int_use:N \l__knot_intersections_int/.try}
    \knot_draw_crossing:nVV {\tl_use:N \l__knot_tmpg_tl} \l__knot_tmpa_dim \l__knot_tmpb_dim
    \group_end:
    \endpgfscope
    \tl_use:N \l__knot_node_tl (\l__knot_name_tl \c_space_tl \int_use:N \l__knot_intersections_int) at (\l__knot_tmpa_dim, \l__knot_tmpb_dim) {};
  }
}

\cs_generate_variant:Nn \knot_intersections:nn {VV}
\prg_new_conditional:Npnn \knot_test_endpoint:N #1 {p,T,F,TF}
{
  \dim_compare:nTF
  {
    \dim_abs:n {\pgf@x - \tl_item:Nn #1 {1}}
    +
    \dim_abs:n {\pgf@y - \tl_item:Nn #1 {2}}
    <
    \l__knot_tolerance_dim
  }
  {
    \prg_return_true:
  }
  {
    \prg_return_false:
  }
}
\prg_new_protected_conditional:Npnn \knot_test_endpoint:nn #1#2 {T,F,TF}
{
  \spath_get:nnN {knot #1} {#2} \l__knot_tmpd_tl
  \knot_test_endpoint:NTF \l__knot_tmpd_tl
  {
    \prg_return_true:
  }
  {
    \prg_return_false:
  }
}

\cs_generate_variant:Nn \knot_test_endpoint:nnT {VnT,vnT}
\cs_generate_variant:Nn \knot_test_endpoint:nnF {VnF,vnF}
\cs_generate_variant:Nn \knot_test_endpoint:nnTF {VnTF,vnTF}
\cs_new_nopar:Npn \knot_draw_crossing:nnn #1#2#3
{
  \group_begin:
  \pgfscope
  \clip (#2, #3) circle[radius=\l__knot_clip_radius_dim];

  \tl_set:Nn \l_tmpa_tl {knot~ diagram/every~ strand/.try,}
  \tl_if_exist:cT {l__knot_options_ #1}
  {
  \tl_put_right:Nv \l_tmpa_tl {l__knot_options_ #1}
  }
  \tl_put_right:Nn \l_tmpa_tl {,knotbg,line~ width= \tl_use:N \l__knot_clip_width_tl * \pgflinewidth}
  \spath_tikz_path:Vn \l_tmpa_tl {knot #1}

  \endpgfscope

  \pgfscope
  \clip (#2, #3) circle[radius=1.1\l__knot_clip_radius_dim];

  \tl_set:Nn \l_tmpa_tl {knot~ diagram/every~ strand/.try,}
  \tl_if_exist:cT {l__knot_options_ #1}
  {
  \tl_put_right:Nv \l_tmpa_tl {l__knot_options_ #1}
  }
  \tl_put_right:Nn \l_tmpa_tl {,knot~ diagram/only~ when~ rendering/.try,only~ when~ rendering/.try}
  \spath_tikz_path:Vn \l_tmpa_tl {knot #1}

  \endpgfscope
  \group_end:
}

\cs_generate_variant:Nn \knot_draw_crossing:nnn {nVV}
\cs_new_protected_nopar:Npn \knot_split_strands:
{
  \int_gzero:N \l__knot_filaments_int
  \int_step_function:nnnN {1} {1} {\l__knot_strands_int} \knot_split_strand:n
  \int_step_function:nnnN {1} {1} {\l__knot_filaments_int} \knot_compute_nexts:n
}
\cs_new_protected_nopar:Npn \knot_compute_nexts:n #1
{
  \tl_clear_new:c {knot next \tl_use:c {knot previous filament #1}}
  \tl_set:cn {knot next \tl_use:c {knot previous filament #1}} {filament #1}
}
\cs_new_protected_nopar:Npn \knot_split_strand:n #1
{
  \int_set_eq:NN \l__knot_component_start_int \l__knot_filaments_int
  \int_incr:N \l__knot_component_start_int
  \tl_set_eq:Nc \l__knot_tmpa_tl {l__knot_options_strand #1}
  \spath_map_segment_function:nN {knot strand #1} \knot_save_filament:NN
}
\cs_new_protected_nopar:Npn \knot_save_filament:NN #1#2
{
  \tl_case:NnF #1
  {
    \g__spath_moveto_tl
    {
      \int_compare:nT {\l__knot_component_start_int < \l__knot_filaments_int}
      {
        \int_set_eq:NN \l__knot_component_start_int \l__knot_filaments_int
      }
    }
    \g__spath_lineto_tl
    {
      \int_gincr:N \l__knot_filaments_int
      \spath_clear_new:n {knot filament \int_use:N \l__knot_filaments_int}
      \spath_put:nnV {knot filament \int_use:N \l__knot_filaments_int} {path} #2
      \tl_set_eq:cN {l__knot_options_filament \int_use:N \l__knot_filaments_int} \l__knot_tmpa_tl

      \tl_clear_new:c {knot previous filament \int_use:N \l__knot_filaments_int}
      \int_compare:nF {\l__knot_component_start_int == \l__knot_filaments_int}
      {
        \tl_set:cx {knot previous filament \int_use:N \l__knot_filaments_int} {filament \int_eval:n {\l__knot_filaments_int - 1}}
      }
    }
    \g__spath_curvetoa_tl
    {
      \int_gincr:N \l__knot_filaments_int
      \spath_clear_new:n {knot filament \int_use:N \l__knot_filaments_int}
      \spath_put:nnV {knot filament \int_use:N \l__knot_filaments_int} {path} #2
      \tl_set_eq:cN {l__knot_options_filament \int_use:N \l__knot_filaments_int} \l__knot_tmpa_tl

      \tl_clear_new:c {knot previous filament \int_use:N \l__knot_filaments_int}
      \int_compare:nF {\l__knot_component_start_int == \l__knot_filaments_int}
      {
        \tl_set:cx {knot previous filament \int_use:N \l__knot_filaments_int} {filament \int_eval:n {\l__knot_filaments_int - 1}}
      }
    }
    \g__spath_close_tl
    {
      \int_gincr:N \l__knot_filaments_int
      \spath_clear_new:n {knot filament \int_use:N \l__knot_filaments_int}
      \tl_set_eq:NN \l_tmpa_tl #2
      \tl_set:Nx \l_tmpa_tl {\tl_item:Nn #2 {1}\tl_item:Nn #2 {2}\tl_item:Nn #2 {3}}
      \tl_put_right:NV \l_tmpa_tl \g__spath_lineto_tl
      \tl_set:Nx \l_tmpa_tl {\tl_item:Nn #2 {5}\tl_item:Nn #2 {6}}
      \spath_put:nnV {knot filament \int_use:N \l__knot_filaments_int} {path} \l_tmpa_tl
      \tl_set_eq:cN {l__knot_options_filament \int_use:N \l__knot_filaments_int} \l__knot_tmpa_tl
      \tl_clear_new:c {knot previous filament \int_use:N \l__knot_filaments_int}
      \int_compare:nF {\l__knot_component_start_int == \l__knot_filaments_int}
      {
        \tl_set:cx {knot previous filament \int_use:N \l__knot_filaments_int} {filament \int_eval:n {\l__knot_filaments_int - 1}}
      }
      \tl_set:cx {knot previous filament \int_use:N \l__knot_component_start_int} {filament \int_use:N \l__knot_filaments_int}
    }
  }
  {
  }
}
\NewDocumentCommand \redraw { m m }
{
  \tikz@scan@one@point\pgfutil@firstofone #2 \relax
  \tl_put_right:Nn \l__knot_redraws_tl {\knot_draw_crossing:nnn}
  \tl_put_right:Nx \l__knot_redraws_tl {
    {strand #1} {\dim_use:N \pgf@x} {\dim_use:N \pgf@y}
  }
}
\ExplSyntaxOff
\def\pgf@sh@@knotanchor#1#2{%
  \anchor{#2 north west}{%
    \csname pgf@anchor@knot #1@north west\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 north east}{%
    \csname pgf@anchor@knot #1@north east\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 south west}{%
    \csname pgf@anchor@knot #1@south west\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 south east}{%
    \csname pgf@anchor@knot #1@south east\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 north}{%
    \csname pgf@anchor@knot #1@north\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 east}{%
    \csname pgf@anchor@knot #1@east\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 west}{%
    \csname pgf@anchor@knot #1@west\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 south}{%
    \csname pgf@anchor@knot #1@south\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
}
\pgfdeclareshape{knot crossing}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritanchorborder[from=circle]
  \pgf@sh@@knotanchor{crossing}{2}
  \pgf@sh@@knotanchor{crossing}{3}
  \pgf@sh@@knotanchor{crossing}{4}
  \pgf@sh@@knotanchor{crossing}{8}
  \pgf@sh@@knotanchor{crossing}{16}
  \pgf@sh@@knotanchor{crossing}{32}
  \backgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
  }
}
\pgfdeclareshape{knot over cross}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a circle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchorborder[from=rectangle]
  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
  }
  \foregroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
 }
}
\pgfdeclareshape{knot under cross}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a circle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchorborder[from=rectangle]
  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
  }
  \foregroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
 }
}
\pgfdeclareshape{knot vert}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a circle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchorborder[from=rectangle]
  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
 }
}
\pgfdeclareshape{knot horiz}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a circle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchorborder[from=rectangle]
  \foregroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
 }
}
%% 
%% Copyright (C) 2011 by Andrew Stacey <stacey@math.ntnu.no>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  spath3.dtx
%%                                  calligraphy_doc.tex
%%                                  knot_doc.tex
%% and the derived files            spath3.ins,
%%                                  spath3.pdf,
%%                                  spath3.sty,
%%                                  tikzlibrarycalligraphy.code.tex
%%                                  tikzlibraryknots.code.tex
%%                                  calligraphy_doc.pdf
%%                                  knots_doc.pdf
%%                                  README.txt
%% 
%%
%% End of file `tikzlibraryknots.code.tex'.

